Stand Up Indulgent Rendezvous

We consider two mobile oblivious robots that evolve in a continuous Euclidean space. We require the two robots to solve the rendezvous problem (meeting in finite time at the same location, not known beforehand) despite the possibility that one of those robots crashes unpredictably. The rendezvous is stand up indulgent in the sense that when a crash occurs, the correct robot must still meet the crashed robot on its last position. We characterize the system assumptions that enable problem solvability, and present a series of algorithms that solve the problem for the possible cases.

==> old-one_or_two_axis.tex <==

\subsection{Rendez-vous with non-rigid movements}

In this section we present Algorithm~\ref{algo:non-rigid, common distance}, which assume that robots have both axis in common. Robots may have different unit distance and movements are non-rigid.
The different moves of a robots depends on whether it is the left or the right robot, and on its \emph{level}. The level of robot that is at distance $d$ from the other robot (according its own coordinate system), is the integer $i\in\Z$ such that $d\in [2^{-i}, 2^{1-i})$.

\begin{algorithm}[H]
 \KwData{
  $r$ : robot executing the algorithm\\
  $d$ : distance to the other robot 
 }

Let $i\in\mathbb{Z}$ such that $d\in [2^{-i}, 2^{1-i})$\;
\lIf{$i \equiv 0 \mod 3$}{
    move to the middle
}
\lIf{$i \equiv 1 \mod 3$}{
    \emph{left} $\rightarrow$ move to middle ;
    \emph{right} $\rightarrow$ move to other
}
\lIf{$i \equiv 2 \mod 3$}{
    \emph{left} $\rightarrow$ move to other ;
    \emph{right} $\rightarrow$ move to middle
}
 \caption{Rendez-vous with non-rigid movement}\label{algo:non-rigid, common distance}
\end{algorithm}

Let $C$ be any configuration and $d$ is the distance (in the global coordinate system $Z$) between the two robots. Let $x$, resp. $y$, be the distance, in $Z$, traveled by the left robot, resp. the right robot. Since the robots moves toward each other, after executing one round, the distance between the robot becomes $f(d,x,y) = |d - x - y|$.


%%%%%
%%%%%
%%%%%
\begin{lemma}\label{lem:f decreases by fixed distance}
If at least one robots is dictated to move to the middle, then we have $f(d,x,y) \leq d - \min(\delta, d/2)$.
\end{lemma}
\begin{proof}
For fixed $d$, using the symmetry of $f$ (with respect to the second and third argument), we have $f(d,x,y) = g_d(x+y)$ with $g_d: w\mapsto |d - w|$.
We know that the distance traveled by the robots is either 0 (if one crashes) or at least $\min(d/2, \delta)$, but we cannot have $x=y=0$. Also, since at least one robot move to the middle, we have either (i) $x \leq d/2$ and $y\leq d$ or (ii) $x \leq d$ and $y\leq d/2$. Hence the sum $x+y$ is in the interval $[\min(d/2, \delta), 3d/2]$. 

As a convex function, the maximum of $g_d$ is reached at the boundary of its domain
\begin{align*}
    f(d,x,y) = g_d(x+y) &\leq \max(g_d(3d/2), g_d(\min(d/2, \delta)))\\
&\leq \max(d/2, d - \min(d/2, \delta)) =  d - \min(d/2, \delta)
\end{align*}
\end{proof}


%%%%%
%%%%%
%%%%%
\begin{lemma}\label{lem:distance decreases by fixed distance}
From a configuration where robots are at distance $d$ (in $Z$), then, after two rounds, the distance between the robots decreases by at least $\min(\delta, d/2)$.
\end{lemma}
\begin{proof}
From the previous lemma, we know that if at least one robot is dictated to move to the middle, then, after one round, the distance between the robots decreases by at least $\min(\delta, d/2)$. 
Otherwise, we know the level of the left robot is $i_l \equiv 2 \mod 3$ and the level of the right robot is $i_r \equiv 1 \mod 3$. If, after one round, the distance between the robots remains greater than $d - \min(\delta, d/2)$, then the order of the robots has changed (the left robot becomes the right and vice and versa). Moreover, the level of each robot is either the same or is increased by one. In all cases, the right robot (previously the left robot) has now level $i_r' \equiv 2 \mod 3$ or $i_r' \equiv 0 \mod 3$, and moves to the middle, so that after one more round, the distance decreases by at least $\min(\delta, d/2)$.
\end{proof}


%%%%%
%%%%%
%%%%%
\begin{lemma}\label{lem: proof of algo, rigid, congruent, correct}
Assuming rigid movement, no crash, and initially the level of the robots are congruent modulo three, Algorithm~\ref{algo:non-rigid, common distance} solves the SUIR problem.
\end{lemma}

\begin{proof}
Let $i\in\mathbb{Z}$ such that the level of both robots are congruent to $i$ modulo three. Depending on the congruence of $i$ modulo three, three cases are possible: 
\begin{enumerate}
\item \label{d0} $i \equiv 0 \mod 3$. By Algorithm~\ref{algo:non-rigid, common distance}, the rendezvous is achieved. 
\item \label{d1} $i \equiv 1 \mod 3$. By Algorithm~\ref{algo:non-rigid, common distance}, in one round, the levels of the robots are congruent to $i+1 \equiv 2 \mod 3$. We retrieve Case~\ref{d2}. 
\item \label{d2} $i \equiv 2 \mod 3$. By Algorithm~\ref{algo:non-rigid, common distance}, in one round, the levels of the robots are congruent to $i+1 \equiv 0 \mod 3$. We retrieve Case \ref{d0}. 

\end{enumerate}
From the cases above, if none of the two robots crashes, we can deduce that the rendezvous is eventually achieved. 
\end{proof}


%%%%%
%%%%%
%%%%%
\begin{lemma}\label{lem: proof of algo, rigid, crash}
Assuming rigid movement and one robot crashes, Algorithm~\ref{algo:non-rigid, common distance} solves the SUIR problem.
\end{lemma}
\begin{proof}
Let $i$ be the level of the correct robot.
Observe that, by Algorithm~\ref{algo:non-rigid, common distance}, if  $i \equiv 1 \mod 3$ (respectively $i \equiv 2 \mod 3$) then the rendezvous is achieved in one round if the left robot (respectively the right robot) is the one that crashes. 

If $i \equiv 1 \mod 3$ and the right robot crashes then by Algorithm~\ref{algo:non-rigid, common distance}, as the left robot moves to the middle, after one round, the left robot has level $i+1 \equiv 2 \mod 3$. By Algorithm~\ref{algo:non-rigid, common distance}, the left robot moves to join the right robot. Thus the rendezvous is achieved. 

Finally, if $i \equiv 2 \mod 3$ and the left robot crashes then by Algorithm~\ref{algo:non-rigid, common distance}, after two rounds, the right robot has level $i+2 \equiv 1 \mod 3$ (the right robot moves two times to the middle). By Algorithm~\ref{algo:non-rigid, common distance}, the right robot moves to join the other robot. Thus the rendezvous is achieved in this case as well. 

From the cases above, we can deduce that the lemma holds. 
\end{proof}


Now we prove that Algorithm~\ref{algo:non-rigid, common distance} works even if robots have different unit distance.

%%%%%
%%%%%
%%%%%
\begin{theorem}\label{thm: proof of algo, non-rigid}
Algorithm~\ref{algo:non-rigid, common distance} solves the SUIR problem with robots having both axis in common, non-rigid movements and different unit distance.
\end{theorem}
\begin{proof}
Consider a configuration $C$ at round $t$. 

By Lemma~\ref{lem:distance decreases by fixed distance}, the distance between the two robots decreases by at least $\min(\delta, d/2)$ every two rounds. Hence, eventually, robots are at distance smaller than $\delta$ from one another and, from this point in time, movements are rigid.

Assume now that movements are rigid. 
Given a configuration $C$, at round $t$, let $i_r$, resp $i_l$, the level of the right robot, resp. the left robot.
If $i_r \equiv i_l \mod 3$ or if one robot crashes, then robots gather in at most three rounds by Lemma~\ref{lem: proof of algo, rigid, crash}.
Assume now both robots are correct. If both robot are dictated to move to the middle, robots gather in one round. Otherwise, lets consider all the case where either $i_l \equiv 2 \mod 3$ or $i_r \equiv 1 \mod 3$.

 If $i_r \equiv 0 \mod 3$ and $i_l \equiv 2 \mod 3$ at time $t$, then, after one round, the order of the robots changes and the distance between the robots is divided by two (for both robots' views) so that $i_r' \equiv 0 \mod 3$ the  $i_l' \equiv 1 \mod 3$. Hence at time $t+1$ both robots are dictated to move to the middle and complete the rendez-vous at time $t+2$.
 
 If $i_r \equiv 1 \mod 3$ and $i_l \equiv 2 \mod 3$ at time $t$, then, after one round, the order of the robots changes and the distance between the robots remains unchanged so that $i_r' \equiv 2 \mod 3$ the $i_l' \equiv 1 \mod 3$. From there, both robots are dictated to move to the middle and complete the rendez-vous at time $t+2$.
 

If $i_l \equiv 0 \mod 3$ and $i_r \equiv 1 \mod 3$, then, after one round, the order of the robots changes and the distance between the robots is divided by two (for both robots' views) so that $i_r' \equiv 1 \mod 3$ the  $i_l' \equiv 2 \mod 3$. From there, we know using the previous case that the rendez-vous is completed at time $t+3$
\end{proof}



\section{Rendez-vous with Only One Common Axis}

Here we assume the robots only agree on a common North \ie, they have the same $y$-axis.
Under such assumption, the configuration can be symmetric if both robots have the same $y$-coordinate. Indeed, in this case the robots are indistinguishable as they cannot distinguish the right to the left.

When the configuration is not symmetric, we can orient the line joining the two robots and use our previous algorithm to solve the problem. Indeed, if the configuration is not symmetric, let $(x_1, y_1)$ be the coordinates of the northernmost robot, and $(x_2, y_2)$ the coordinates of the other robot ($x_2 < x_1$). Now each robot orient the line joining the two robots with vector $v$ with 
\[
 v = \frac{(|x_1 - x_2|, y_1-y_2)}{\lVert r_{max} - r_{min}\rVert}.
\]
Notice that vector $v$ is invariant up to scaling, translation and does not depend on the orientation of the $x$-axis (because we only use the distance between $x_1$ $x_2$), so both robots can compute $v$ and orient the line in the same way. Like in the proof of Theorem~\ref{thm:1D to 2D}, if robots remains on the same line, the line and its orientation remains invariant.
Hence, the SUIR problem is completed by executing Algorithm~\ref{algo:non-rigid, common distance} on this line.


However, if the configuration is symmetric, the robot can try to remain on the same line to gather like in the previous algorithm, but doing so implies the existence of a configuration where a robot is dictated to move to the other robot. In this symmetric configuration, both robots exchange their position and we obtain the same configuration after one round. This could occur infinitely often without the robots completing the rendez-vous (when both robots are correct).

So, in order to solve this problem, in such configuration, a robot needs to move outside of the line joining the robots.
Our final algorithm is the following. 


If the configuration is symmetric, move to the point that forms, with the two robots, an equilateral triangle. Since two of such point exist, choose the northernmost one.

\begin{algorithm}[H] 
\KwData{
  $r$ : robot executing the algorithm
 }
Let $\{(0,0), (x,y)\}$ be $r$'s local view.\\
\uIf{$y = 0$}{
    move to the point $\left(x/2, \left|\frac{x\sqrt{3}}{2}\right|\right)$
}
\uElse{
    Execute Algorithm~\ref{algo:non-rigid, common distance}
}
 \caption{Rendez-vous with non-rigid movement}\label{algo:one common axis}
\end{algorithm}

\begin{theorem}\label{thm: proof of algo, one axis, non-rigid}
Algorithm~\ref{algo:one common axis} solves the SUIR problem with non-rigid movements and robots having only one common axis and different unit distance.
\end{theorem}

\begin{proof}
If the configuration is not symmetric, then, by executing Algorithm~\ref{algo:non-rigid, common distance}, the obtained configurations remains asymmetric and the theorem follows from Theorem~\ref{thm: proof of algo, non-rigid}.

Consider now that the initial configuration $C$ is symmetric. 
If one robot crashes, then, after one round, the configuration is asymmetric and we retrieve the previous case.
If both robots are correct and reach their destination, the rendez-vous is completed in one round. If robots are stopped before reaching their destinations, two cases can occur. Either they are stopped after traveling different distances or they are stopped at the same $y$-coordinate. In the former case, the obtained configuration is asymmetric and we retrieve the first case. In the latter, the configuration remains symmetric, by the distance between the two robots decreases by at least $\frac{2\delta}{\sqrt{2}}$ as illustrated in Figure~\ref{fig:moving to the vertex of the equilateral triangle}. Hence, at each round either robots complete the rendez-vous, reach an asymmetric configuration or come closer by a fixed distance. Since the latter case cannot occurs infinitely often, one of the other case occurs at least once and the rendez-vous is completed in finite amount of rounds.


\begin{figure}[h]
    \centering
\begin{tikzpicture}

\draw[dashed] (0,0) -- (0:3);

\node[robot] (a) at (0:0) {};
\node[robot] (b) at (0:3) {};
\node[dest] (c) at (60:3) {};



\draw[] (0,0) -- (150:0.5);
\draw[] (60:0.9) -- ($(60:0.9)+(150:0.5)$);
\draw[<->, line width = 0.8pt] (150:0.4) -- ($(60:0.9)+(150:0.4)$);

\node[opacity=0, fill=white, inner sep = 1pt, text opacity=1] at ($(60:0.45)+(150:0.6)$) {$\delta$};


\draw[] (60:0.9) -- ($(60:0.9)+(-90:1.28)$);
\draw[] (0,0) -- ($(-90:0.5)$);
\draw[<->, line width = 0.8pt] (-90:0.3) -- ($(60:0.9)+(-90:1.08)$);

\node[opacity=0, fill=white, inner sep = 1pt, text opacity=1] at (0.2,-0.9) {$\frac{\delta}{\sqrt{2}}$};



\draw[] (0:3) -- ($(0:3)+(30:0.5)$);
\draw[] ($(0:3) + (120:0.9)$) -- ($(0:3)+(120:0.9)+(30:0.5)$);
\draw[<->, line width = 0.8pt] ($(0:3)+(30:0.5)$) -- ($(0:3)+(120:0.9)+(30:0.4)$);

\node[opacity=0, fill=white, inner sep = 1pt, text opacity=1] at ($(0:3)+(120:0.45)+(30:0.6)$) {$\delta$};


\draw[] ($(0:3) + (120:0.9)$) -- ($(0:3)+(120:0.9)+(-90:1.28)$);
\draw[] (0:3) -- ($(0:3)+(-90:0.5)$);
\draw[<->, line width = 0.8pt] ($(0:3)+(-90:0.3)$) -- ($(0:3)+(120:0.9)+(-90:1.08)$);

\node[opacity=0, fill=white, inner sep = 1pt, text opacity=1] at (2.8,-0.9) {$\frac{\delta}{\sqrt{2}}$};

\draw[->, line width = 1.pt] (a) -- (c);
\draw[->, line width = 1.pt] (b) -- (c);


\end{tikzpicture}
    \caption{Robots moving to the third vertex of the equilateral triangle}
    \label{fig:moving to the vertex of the equilateral triangle}
\end{figure}

\end{proof}



==> old-reduction.tex <==

QB: le theorem n'est plus utile tel quel. il faut qu'il soit plus général.
\begin{theorem}\label{thm:1D to 2D}
Suppose there exists an algorithm solving the SUIR problem where robots are restricted to a one-dimensional space and agree on its the orientation. Then, there exists an algorithm solving the SUIR problem on the two-dimensional space, where robots agree on both axis.
\end{theorem}
\begin{proof}

\begin{figure}
    \centering
\begin{tikzpicture}
\draw[->, line width=1.5pt] (0,0) -- (0,1);
\draw[->, line width=1.5pt] (0,0) -- (1,0);


\draw[] (-2, 1.5-2.4*0.9/1.6) -- 
(3, 2.4+1*0.9/1.6);

\draw[dashed] (-0.5, 0.5*1.6/0.9) -- 
(0, 0);

\draw[->, line width=1.5pt] (-0.55, 0.55*1.6/0.9) -- (0.4,1.5);

\node[robot, minimum width=2.5pt] (a) at (0,0) {};
\node[robot, minimum width=2.5pt] (a) at (-0.55, 0.55*1.6/0.9) {};
\node[opacity=1, fill=white, inner sep = 1pt, text opacity=1] at (-0.75, 1.25) {$O$};
\node[opacity=1, fill=white, inner sep = 1pt, text opacity=1] at (-0.25, 1.55) {$v$};

\node[robot] (a) at (-1.5, 1.5-1.9*0.9/1.6) {};
\node[robot] (b) at (2,2.4) {};


\node[opacity=1, fill=white, inner sep = 1pt, text opacity=1] at (-1.55, .8) {$r_1$};
\node[opacity=1, fill=white, inner sep = 1pt, text opacity=1] at (2.1, 2) {$r_2$};

\node[opacity=0, text opacity=1] at (0.2,-0.6) {};
\end{tikzpicture}
    \caption{One-dimensional coordinate system $(O, v)$. The coordinate system remains invariant as long as robots stays one the line and are not gathered.}
    \label{fig:illustration of the 1D coodinate system}
\end{figure}


 Let $A_1$ be an algorithm solving the SUIR problem where robots are restricted to a one-dimensional space. The proof is by construction.
We define algorithm $A_2$ executed by robots on the two-dimensional space.

First, if the local view of a robot is $\{(0,0)\}$, then $A_2$ output $(0,0)$. Otherwise, when a robot $r$ has a local view $\{(0,0), (x,y)\}$, it can compute the corresponding coordinates on the axis formed by the two robots. 
\[
w = \left\{\begin{array}{ll}
    \sqrt{x^2+y^2}&\text{if $x>0$ or $x=0\land y>0$}\\
    -\sqrt{x^2+y^2}&\text{otherwise}\\
\end{array}\right.
\]
$|w|$ corresponds to the distance between the two robots in the global coordinate system $Z$, times the unit distance of robot $r$.
Then, the robot computes its destination target $p = A_1(\{0, w\}) \in \R$ on the axis using algorithm $A_1$.
This destination is finally converted into a destination $(x_p, y_p)$ on the plane 
 \[
 \left\{\begin{array}{l}
    x_p = p \cos(\varphi)\\
    y_p = p \sin(\varphi)\\
\end{array}\right.
 \]
 Where $\varphi\in\left(-\frac{\pi}{2}, \frac{\pi}{2}\right]$ is the angle of the line formed by the two robots 
 \[
 \varphi = \left\{
 \begin{array}{ll}
       \arctan\left(\frac{y}{x}\right)& \text{if $x\neq 0$} \\
      \frac{\pi}{2}&\text{Otherwise} 
 \end{array}\right.
 \]
 
% Je pensait mettre une fleche dessus mais finalement non
\newcommand{\vv}{v}

Given any local view $\{r_{min}, r_{max}\}$, where $r_{min} < r_{max}$, we can define the unit vector $\vv_r$ that orients the line joining the two robots as follows 
\[
 \vv_r = \frac{r_{max} - r_{min}}{\lVert r_{max} - r_{min}\rVert}.
\]
Notice that $\vv_r$ depends only on the transformation function of $r$ and on the angle $\phi$ of the line. Since the robots stay on the same line, $\varphi$ remains constant over time, and since the transformation function of $r$ also does not change over time, then $\vv_r$ does not change over time. Moreover, if the two robots $r$ and $r'$ agree on both axis, then $\vv_r = \vv_{r'}$ and the robots agree on the orientation of the line.

Our algorithm $A_2$ can be described using vector $v$. Using the same notation as before, we see that $w$ is such that the local view of $r$ is $\{(0,0), w\vv_r\}$ and the destination of $r$ is $(x_p, y_p) = p\vv_r$. 
In the global coordinate system, the destination of $r$ is $r + h_r^{-1}(p\vv_r)$.
By construction, the destination of each robot is on the line $L$ joining the two robots, so $L$ and its orientation (vector $\vv_r$) remains invariant during the whole execution.

Let $Z$ be the coordinate system we use for the analysis and let $O$ be a point on the line $L$ and $\vv_{global}$ a unit vector that orients line $L$. Then $(O, \vv_{global})$ is an oriented one-dimensional global coordinate system of the line $L$ (not accessible to the robots).
Let $m$ be the mapping of coordinates in $Z$ to coordinates in $(O, \vv)$.
\[
m(x,y) = a \qquad \text{iif $(x,y) = O + a\vv_{global}$}
\]
We can extend the function $m$ to configurations as follows: $m(C) = \{m(r)\;|\; r\in C\}$. We also define the transformation function $\overline{h}_{r}$ of a robot $r$ on the line by $\overline{h}_{r}(a) = b$ iif $r+a\vv_{global} = r+b\vv$.


Now consider a configuration $C=\{r_1, r_2\}$ such that $r_1 = O + a_1\vv_{global}$ and $r_2 = O + a_2\vv_{global}$. Then, we have $m(C) = \{a_1, a_2\}$.
On one hand, if both robots in $m(C)$ are activated and execute algorithm $A_1$, we obtain by definition the configuration 
\[
B = \{a_1 + \overline{h}_{r_1}(p_1), a_2 + \overline{h}_{r_2}(p_2)\}
\]
Where $p_i = A_1(\{0, \lambda_i(a_j - a_i\})$, with $i = 1, 2$ and $j = 2-i$.

On the other hand, the destination, in $\R^2$, of $r_i$ is $O+a_i\vv_{global}+\overline{h}_{r_i}^{-1}(p_i)\vv_{global}$ for $i=1, 2$.
The obtained configuration after executing $A_2$ on $C$ is $C'$:
\[
C' = \{O+(a_1+\overline{h}_{r_i}(p_1))\vv_{global}, O+(a_2+\overline{h}_{r_i}(p_2))\vv_{global}\}
\]

We observe that $B = m(C')$ \ie, if $C\overset{A_1}{\rightarrow} C'$, then $m(C)\overset{A_2}{\rightarrow} m(C')$. Notice that this is true even if $C$ is a singleton as in this case $A_2$, like $A_1$, dictates the robots not to move.
If a single robot is activated or, if robots are stopped before reaching their destination, one can show a similar equivalence.

Consider an arbitrary execution $C_0,C_1,\ldots$ of $A_2$. As illustrated in Figure~\ref{fig:1D to 2D diagram}, we saw that the sequence $m(C_0), m(C_1), \ldots$ is an execution of $A_1$, so that there exists a point $p\in \R$ and a round $t$ such that, for all $t'\geq t$, $m(C_{t'}) = \{p\}$. This implies that $C_{t'} = \{ 0+p\vv \}$, so that $A_2$ solves the SUIR problem.

\begin{figure}
    \centering
    \begin{tikzpicture}
      \matrix (m) [matrix of math nodes,row sep=3em,column sep=4em,minimum width=2em]
      {
         C_0 & C_1 & C_2 & \phantom{C_3}\\
         m(C_0) & m(C_1) & m(C_2) & \phantom{C_3}\\};
      \path[-stealth]
        (m-1-1) edge node [left] {$m$} (m-2-1)
                edge node [above] {$A_2$} (m-1-2)
        (m-2-1.east|-m-2-2) edge node [above] {$A_1$} (m-2-2)
        (m-1-2) edge node [left] {$m$} (m-2-2)
        
        (m-1-2) edge node [above] {$A_2$} (m-1-3)
        (m-2-2) edge node [above] {$A_1$} (m-2-3)
        (m-1-3) edge node [left] {$m$} (m-2-3)
                
        (m-1-3) edge [dashed,-] (m-1-4)
        (m-2-3) edge [dashed,-] (m-2-4);
    \end{tikzpicture}
    \caption{Diagram showing the link between the execution of $A_1$ in the one-dimensional space and the execution of $A_2$ in the two-dimensional space.}
    \label{fig:1D to 2D diagram}
\end{figure}


\end{proof}

==> old_proofs.tex <==



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  Vieux algo
%






\section{Rendez-vous on a continuous line with different unit distance}


Algorithm $\mathcal{A}$ executed by robot $r$. \\
Let $d$ the distance between the two robot according to $r$'s unit of distance.
\begin{itemize}
    \item[1)] If $d > 1$, the target destination is the middle of the two robots.
    \item[2)] If $d \leq 1$. If $r$ is the right robot, the target destination is the position of the other robot. Otherwise, the target destination is the point located one unit on the right of the other robot.
\end{itemize}

\begin{figure}[h]
    \centering
\begin{tikzpicture}
\draw[->] (-1,0) -- (3,0);
\node[robot] (a) at (0,0) {};
\node[robot] (b) at (2,0) {};
\node[dest] (m) at (1,0) {};
\node[opacity=0, text opacity=1] at (0,-0.5) {$>1$};
\node[opacity=0, text opacity=1] at (2,-0.5) {$>1$};

\path (a) edge[bend left=60,->,>=stealth'] node [left] {} (m);
\path (b) edge[bend right=60,->,>=stealth'] node [left] {} (m);
\end{tikzpicture}~~~~~~
\begin{tikzpicture}
\draw[->] (-1,0) -- (3,0);
\node[robot] (a) at (0,0) {};
\node[robot] (b) at (2,0) {};
\node[dest] (m) at (1,0) {};
\node[opacity=0, text opacity=1] at (0,-0.5) {$>1$};
\node[opacity=0, text opacity=1] at (2,-0.5) {$\leq 1$};

\path (a) edge[bend left=40,->,>=stealth'] node [left] {} (m);
\path (b) edge[bend right=70,->,>=stealth'] node [left] {} (a);
\end{tikzpicture}

\begin{tikzpicture}
\draw[->] (-1,0) -- (4.2,0);
\node[robot] (a) at (0,0) {};
\node[robot] (b) at (1.3,0) {};
\node[dest] (r) at (3.5,0) {};
\node[opacity=0, text opacity=1] at (0,-0.5) {$\leq 1$};
\node[opacity=0, text opacity=1] at (1.3,-0.5) {$\leq 1$};

\path (a) edge[bend left=55,->,>=stealth'] node [left] {} (r);
\path (b) edge[bend right=35,->,>=stealth'] node [left] {} (a);
\end{tikzpicture}~~~~~~
\begin{tikzpicture}
\draw[->] (-1,0) -- (4.2,0);
\node[robot] (a) at (0,0) {};
\node[robot] (b) at (1.3,0) {};
\node[dest] (m) at (1.3/2,0) {};
\node[dest] (r) at (3.5,0) {};
\node[opacity=0, text opacity=1] at (0,-0.5) {$\leq 1$};
\node[opacity=0, text opacity=1] at (1.3,-0.5) {$> 1$};

\path (a) edge[bend left=55,->,>=stealth'] node [left] {} (r);
\path (b) edge[bend right=40,->,>=stealth'] node [left] {} (m);
\end{tikzpicture}

    \caption{The four possible configurations, depending on how each robot perceives its distance with the other robot}
    \label{fig:four possible configurations}
\end{figure}


\begin{theorem}
$\mathcal{A}$ solves the rendez-vous problem in FSYNC with up to one crash fault.
\end{theorem}
\begin{proof}
If the left robot crashes, the right robot halves its distance with the other robot each round until its distance is at most one unit. Then, the right robot executes line 2) of the algorithm and the robots gather.

If the right robot crashes, the left robot halves its distance with the other robot each round until its distance is at most one unit. Then, the left robot executes line 2) of the algorithm and ends up on the right of the other robot, at distance one. It then executes line 2) of the algorithm and the robots gather.

Now assume no robot crashes.
If the configuration is in $C(>1,>1)$, both robots execute line 1) of the algorithm and gather in one round.
If the configuration is in $C(\leq 1,>1)$. Then, after one round, the obtained configuration is in $C(>1,>1)$. Indeed, the robots increased their distance, and are in the reversed order so the configuration is in $C(>1,*)$ and, since the right robot moved to the left and the left robot moved at one unit to the right of it, the right robot is now at distance at least one unit from the other robot.
If the configuration is in $C(\leq 1,\leq 1)$, then, after one round the configuration is either in $C(>1,>1)$ or in $C(\leq 1, >1)$. In both case, the robots eventually gather.
If the configuration is in $C(> 1,\leq 1)$, then, after one round the configuration is either in $C(\leq 1,>1)$ or in $C(\leq 1, \leq 1)$. In both case, the robots eventually gather.
\end{proof}








\section{Rendez-vous on a discrete line}

common distance units.

Observation: If an algorithm solves the problem on a directed line, then there is an algorithm that solves the problem on the plane. 

Consider a unidimensional setting. Also, for the time being, consider robots are only at (full) unit distance locations. An algorithm could be as follows : 

Algorithm $\mathcal{A}$ executed by robot $r$. \\
Let $d$ the distance between the two robot.
\begin{itemize}
    \item If $d=1$. If $r$ is the left robot, move right by two units. Otherwise, move left by one unit.
    \item If $d \geq 2$. If $r$ is the left robot, move right by two $\left\lceil \frac{d}{2} \right\rceil$ units. Otherwise, move left by $\left\lfloor \frac{d}{2} \right\rfloor$ units.
\end{itemize}

\begin{theorem}
$\mathcal{A}$ solves the rendez-vous problem in FSYNC with up to one crash fault.
\end{theorem}
\begin{proof}
-

\includegraphics[]{PastedGraphic-1.png}

If none of the robots are crashed, moving to the same half location gathers the robots. If the initial distance is one, it becomes 2 so after one more step, gathering is achieved.

If the left robot is crashed, the right robot halves the distance until it reached one, then goes to the left robot position.

\includegraphics[]{PastedGraphic-2.png}

 If the right robot is crashed, the left robot gets closer then passes the initial right robot by the right, and we are back to the previous situation.
\includegraphics[]{PastedGraphic-3.png}

If the robots are not on (full) units initially, they first move to it. However, if the other robot is not at a (full) unit distance, then consider it to be at the closest unit distance when running the algorithm. 
\end{proof}




%
% Vieille preuve fausse!
%

\section{Impossibility of Rendez-vous with non-rigid movements and different unit distance in 1D}

Idea:
We know there is a view $V_l$ where the a robot is dictated to move to the other robot. Assume without loss of generality that the left robot does so.
If there exists a view $V_r$ such that the right robot move to the other or to its left, then, in any distinct configuration $C$, the adversary can choose the distance unit $\lambda_r$ for the right robot, resp. $\lambda_l$ for the left robot, so that the right robot sees view $V_r$, resp. the left robot sees view $V_l$. The adversary can stopped the right robot so that it end up on the previous location of the left robot. Thus, both robots swap their positions and this can occur infinitely often.
So there is no view such that the right robot is dictated to move to the other robot or on its left

==> open.tex <==
Similarly, one can design a luminous robot algorithm with three colors in SSYNC.

\begin{algorithm}[H]
 \KwData{
  $r$ : robot executing the algorithm\\
  $o$ : other robot\\
  $c(i)$ : color of robot $i$, either 0, 1, or 2\\
 }

\lIf{$c(r)=c(o)$}{
    $c(r) := c(r)+1 \mod 3$;
    move to the middle
}
\lIf{$c(r)=c(o)+1 \mod 3$}{
    move to other
}
\lIf{$c(r)=c(o)-1 \mod 3$}{
    $c(r) := c(r)-1 \mod 3$;
}
 \caption{Rendez-vous with Luminous robots in SSYNC}\label{algo:luminous SSYNC}
\end{algorithm}

\begin{lemma}
When there is no crash and moves are rigid, Algorithm~\ref{algo:luminous SSYNC} solves gathering in SSYNC.
\label{lem:nocrash_luminous}
\end{lemma}

\begin{proof}
If robots share the same position, no robot moves.

If the lights have the same color, either both robots are activated and join in the middle, or one robot is activated and goes to the middle and change its color. 
\textbf{ST: this part is incorrect.}
If the light colors are different, one robot goes to the other robot that does not move. 
\end{proof}

\begin{lemma}
When there is one crash and moves are rigid, Algorithm~\ref{algo:luminous SSYNC} solves gathering in SSYNC.
\label{lem:crash_luminous}
\end{lemma}

\begin{proof}
Without loss of generality, suppose $r_2$ is crashed and $r_1$ is not crashed.
If robots share the same position, no robot moves.

If the lights are the same color, $r_1$ goes to the middle and changes its color.
If the lights have different color, then two cases can occur:
\begin{enumerate}
\item $c(r_1)=c(r_2)+1 \mod 3$, then $r_1$ joint $r_2$
\item $c(r_1)=c(r_2)-1 \mod 3$, then $r_1$ changes its color so that the first case occurs. 
\end{enumerate}
In any case, rendez-vous is eventually achieved.
\end{proof}

\begin{theorem}
Algorithm ~\ref{algo:luminous SSYNC} solves SUIR in SSYNC, even if the robot colors in the initial configuration are arbitrary.
\end{theorem}

\begin{proof}
In the case of non-rigid moves, one can observe that instead of joining the other robot or the middle point, a correct robot approaches the other robot by at least $\delta$. Thus, if the robots do not join, at every round, the distance between the robots decreases by a constant strictly positive distance. Eventually, the distance between the two robots becomes smaller than $\delta$, and rigid moves can be assumed.
Then, by lemmas~\ref{lem:nocrash_luminous} and \ref{lem:crash_luminous}, rendez-vous is achieved. Note that the lemmas hold irrelevant of the initial colors of both robots. Hence, the theorem holds.
\end{proof}

==> triangle-equilateral.tex <==
\begin{tikzpicture}

\draw[dashed] (0,0) -- (0:3);

\node[robot] (a) at (0:0) {};
\node[robot] (b) at (0:3) {};
\node[dest] (c) at (60:3) {};



\draw[] (0,0) -- (150:0.5);
\draw[] (60:0.9) -- ($(60:0.9)+(150:0.5)$);
\draw[<->, line width = 0.8pt] (150:0.4) -- ($(60:0.9)+(150:0.4)$);

\node[opacity=0, fill=white, inner sep = 1pt, text opacity=1] at ($(60:0.45)+(150:0.6)$) {$\delta$};


\draw[] (60:0.9) -- ($(60:0.9)+(-90:1.28)$);
\draw[] (0,0) -- ($(-90:0.5)$);
\draw[<->, line width = 0.8pt] (-90:0.3) -- ($(60:0.9)+(-90:1.08)$);

\node[opacity=0, fill=white, inner sep = 1pt, text opacity=1] at (0.2,-0.9) {$\frac{\delta}{\sqrt{2}}$};



\draw[] (0:3) -- ($(0:3)+(30:0.5)$);
\draw[] ($(0:3) + (120:0.9)$) -- ($(0:3)+(120:0.9)+(30:0.5)$);
\draw[<->, line width = 0.8pt] ($(0:3)+(30:0.5)$) -- ($(0:3)+(120:0.9)+(30:0.4)$);

\node[opacity=0, fill=white, inner sep = 1pt, text opacity=1] at ($(0:3)+(120:0.45)+(30:0.6)$) {$\delta$};


\draw[] ($(0:3) + (120:0.9)$) -- ($(0:3)+(120:0.9)+(-90:1.28)$);
\draw[] (0:3) -- ($(0:3)+(-90:0.5)$);
\draw[<->, line width = 0.8pt] ($(0:3)+(-90:0.3)$) -- ($(0:3)+(120:0.9)+(-90:1.08)$);

\node[opacity=0, fill=white, inner sep = 1pt, text opacity=1] at (2.8,-0.9) {$\frac{\delta}{\sqrt{2}}$};

\draw[->, line width = 1.pt] (a) -- (c);
\draw[->, line width = 1.pt] (b) -- (c);
\end{tikzpicture}
